AdvisorQA: Towards Helpful and Harmless Advice-seeking Question Answering with Collective Intelligence

As the integration of large language models into daily life is on the rise, there is a clear gap in benchmarks for advising on subjective and personal dilemmas. To address this, we introduce AdvisorQA, the first benchmark developed to assess LLMs' capability in offering advice for deeply personalized concerns, utilizing the LifeProTips subreddit forum. This forum features a dynamic interaction where users post advice-seeking questions, receiving an average of 8.9 advice per query, with 164.2 upvotes from hundreds of users, embodying a collective intelligence framework. Therefore, we've completed a benchmark encompassing daily life questions, diverse corresponding responses, and majority vote ranking to train our helpfulness metric. Baseline experiments validate the efficacy of AdvisorQA through our helpfulness metric, GPT-4, and human evaluation, analyzing phenomena beyond the trade-off between helpfulness and harmlessness. AdvisorQA marks a significant leap in enhancing QA systems for providing personalized, empathetic advice, showcasing LLMs' improved understanding of human subjectivity.

==> Text/1_Introduction.tex <==


\input{Resource/Intro.tex}

Large language models (LLMs)~\citep{openai2023gpt, touvron2023llama} have significantly enhanced \textit{objective decision-making} in healthcare~\citep{moor2023foundation, arora2023promise}, science~\citep{kung2023performance}, and coding~\citep{ni2023lever}. With this progress, there has been an emphasis on developing benchmarks that assess the helpfulness of LLMs~\citep{hendrycks2020measuring, cobbe2021training, hwang2022multi, ye2023flask}. However, there is a pronounced need for AI to \textbf{advise} \textit{subjective decision-making} regarding deeply personalized issues that individuals face~\citep{casper2023open, kasneci2023chatgpt}. The complex nature of advice on human problems involves various subjective considerations, which are not sufficiently addressed by purely objective evaluations~\citep{bolotova2022non, bolotova-baranova-etal-2023-wikihowqa}.

%P2
% To this end, we introduce AdvisorQA, a benchmark for Advice-seeking Question Answering, built on the millions-user scale subreddit forum LifeProTips\footnote{\url{https://www.reddit.com/r/LifeProTips/}} dedicated to advising on personal daily concerns. The questions in AdvisorQA are significantly more complex than those in previous tasks. Each session's advice-seeking question, as shown in Figures~\ref{fig:Intro} and~\ref{fig:construction}, are intensely personal, capable of generating a broad spectrum of subjective viewpoints.
% This complexity is evidenced by the significantly high average token length detailed in Table~\ref{tab:stats} and the wide variety of topic distributions from A to B, showcased in Figure~\ref{fig:Q_vis}. 
% Furthermore, the rich diversity of subjective viewpoints produces various responses for each question, demonstrating minimal information redundancy, as shown in Tables~\ref{tab:stats} and \ref{tab:stats2}. 
% Therefore, AdvisorQA is distinctly different from previous benchmarks by allowing a wide range of subjective opinions on very personal issues.

To this end, we introduce AdvisorQA, a benchmark for Advice-seeking Question Answering, built on the millions-user scale subreddit forum LifeProTips\footnote{\url{https://www.reddit.com/r/LifeProTips/}}, dedicated to advising on personal daily concerns. Within LifeProTips, as exemplified in Figure~\ref{fig:construction}, each session comprises user-submitted personal dilemmas, various advisory responses, and subsequent discussions and upvotes indicating the majority preference.  We have crawled a total of 10,350 sessions and established a benchmark that evaluates the performance of LLM-generated advice.
% We have crawled a total of 10,350 sessions and established a benchmark that evaluates the performance of LLM-generated advice based on its ranking among existing responses, as illustrated in Figure~\ref{fig:Intro}.

The advice-seeking questions in AdvisorQA are significantly more complex than previous \textit{objective} goal benchmarks, such as MMLU~\citep{mmnlu-2022-massively}, GSM8K~\citep{cobbe2021training}, and Flask~\citep{ye2023flask}. As shown in Figures~\ref{fig:Intro} and~\ref{fig:construction}, each question is profoundly personal and possesses the capacity to engage a broad spectrum of \textit{subjective} viewpoints. This complexity is evidenced by the wide variety of topic distributions, from social dilemmas to career consulting, showcased in Figure~\ref{fig:Q_vis}. This personal narrative leads to a significantly high average 75.2 token length only in questions. Moreover, the rich diversity of subjective viewpoints yields a variety of response types for each question, showing little redundancy in the content of the responses.

Annotating preferable advice on deeply personal experiences presents formidable challenges~\citep{krishna-etal-2021-hurdles}. When evaluating the helpfulness of highly subjective advice, relying solely on a few annotators' preferences could introduce their biases~\citep{casper2023open, weerasooriya-etal-2023-subjective}. Hence, collaborative brainstorming among individuals with diverse backgrounds is necessary~\citep{sandri-etal-2023-dont, fleisig-etal-2023-majority}. Therefore, we adopted the advice rankings voted by around \textbf{164.2} average users in each session, which is considered as a form of \textbf{Collective Intelligence}~\cite{fan-etal-2019-eli5, yang-etal-2023-rumor}. This novel approach enabled us to complete our benchmark, positioning AdvisorQA as a pioneering tool for harnessing collective intelligence in evaluating subjective advice, as illustrated in Figure~\ref{fig:Intro}.

% 그다음문단 베이스라인 요약하여 얘기

Given the allowance for a wide range of subjective opinions in AdvisorQA, information similarity metrics for assessing helpfulness are less practical than objective benchmarks~\citep{zha-etal-2023-alignscore, min-etal-2023-factscore}. Therefore, we designed a helpfulness metric through the Plackett-Luce (PL) model~\citep{plackett1975analysis}, widely used for reward modeling to rank candidate responses. The results showed that even smaller-scale models (1.4B) could predict the ground truth advice ranking in the test set more accurately than GPT-4 (>> 175B). Beyond numerical scores, further analysis revealed that the PL model sensitively detects \textit{empathic and practical} elements. However, we find our helpfulness metric failed to capture ethical considerations, leading us to employ the LifeTox moderator~\citep{kim2023lifetox} from the same subreddit source as a harmlessness metric. Through these metrics, we conducted an in-depth analysis of the baselines using two orthogonalized views: \textit{helpfulness} and \textit{harmlessness}.

Baseline experiments measured the advising performance of various LLMs and analyzed how models evolved when trained on AdvisorQA using widely used alignment methods: PPO~\citep{schulman2017proximal} and DPO~\citep{rafailov2023direct}. The results showed an increase in helpfulness from the perspectives of the PL model, GPT-4, and human evaluation, affirming the validity of the AdvisorQA dataset. However, while PPO models tended to become unsafe, DPO models showed a safer progression. Further analysis revealed that DPO's safety stemmed from its tendency to follow demonstrations and produce strictly written advice. In contrast, PPO's capacity to generate more empathic and diverse advice indicates potential synergy with controllable text generation in future researches~\citep{liu-etal-2021-dexperts, kim-etal-2023-critic, deng-raffel-2023-reward}.

The new benchmark AdvisorQA serves as a valuable resource for advancing everyday QA systems that provide in-depth, empathetic, and practical advice based on deeply personalized experiences. By leveraging collective intelligence to evaluate various subjective opinions and through baseline experiments, we have confirmed the dataset's validity and shed light on the characteristics of existing alignment methodologies in subjective domains. These analyses suggest a broad potential to facilitate research in evaluating and training systems for daily neural advisors.

% Contribution 요약은 논문 길이에 따라 빠져도 or 조절되면 좋을 것 같습니다.
% The main contributions of this paper are summarized as threefolds;

% \begin{enumerate}
% \item We propose a novel benchmark, AdvisorQA: Advice-seeking Question Answering, for pioneering personalized and subjective areas.

% \item AdvisorQA aims to advance subjective domain metrics evaluation and uses training set advice rankings to predict test set rankings, offering a new approach to evaluate subjective viewpoints.

% \item The second objective of AdvisorQA is to train LLMs as neural advisors, assessing their helpfulness and harmlessness through baseline experiments, thereby establishing a benchmark for their deployment in everyday life scenarios.

% \item Something closing mention with experimental results?

% \end{enumerate}


% 화란님 이 두 문단은 제가 baseline으로 요약해서 다시 적겠습니다. Task 1,2구조에서 -> Eval & Baseline으로 (GOOD :) )
% With AdvisorQA's content and the collective intelligence in advice rankings, we pursue two ambitious goals. First, we aim to \textbf{evaluate the evaluation pipelines for AdvisorQA}.
% % (suggestion) With AdvisorQA, we formulate two benchmark tasks: 1) ranking prediction of advice, 2) training a helpful and safe neural advisor that is aligned with the crowd's preference values.
% In the era of long-form QA, the importance of evaluation methods is growing, leading to the development of innovative evaluation methods like LongEval~\citep{krishna-etal-2023-longeval}, AlignScore~\citep{zha-etal-2023-alignscore}, and FactScore~\citep{min-etal-2023-factscore} for tasks with objective missions. Nonetheless, progress in subjective domains, hindered by the limitations of n-gram similarity in contexts with diverse opinions, has been slower~\citep{krishna-etal-2021-hurdles}. In AdvisorQA, which reflects a range of preference values, we propose using training set advice rankings to identify the majority values in adopted forums. We then evaluate how effectively these values predict the unseen test set rankings. This benchmark offers a valuable testing ground for subjective evaluation methodologies, significantly advancing our capacity to understand and evaluate diverse, subjective viewpoints.

% The second goal involves \textbf{training LLMs as neural advisors in various personalized scenarios}. Here, we evaluate their helpfulness and harmlessness in safely addressing various concerns. Baseline experiments were conducted using Proximal Policy Optimization (PPO)~\citep{schulman2017proximal} and Direct Preference Optimization (DPO)~\citep{rafailov2023direct}, recognized as standards for aligning with human values. These experiments enable us to analyze the effectiveness of each Reinforcement Learning (RL) strategy in the context of personal and subjective advice-seeking question answering. Through this analysis, AdvisorQA emerges as a benchmark for preparing LLMs for deployment in services integral to daily life.



% Evaluating advice on deeply personal experiences presents formidable challenges~\citep{krishna-etal-2021-hurdles, casper2023open, weerasooriya-etal-2023-subjective}. Each question can elicit a range of subjective opinions, necessitating an assessment approach that extends beyond a limited number of annotators to collaborative brainstorming among individuals with diverse backgrounds~\citep{sandri-etal-2023-dont, fleisig-etal-2023-majority}. Furthermore, managing ethical issues emerging in the problem-solving process is crucial~\citep{lee-etal-2023-square, hendrycks2023aligning}. To navigate this complexity, we utilized the millions-user scale subreddit forum LifeProTips, a dynamic platform where individuals share advice on personal matters and engage in thorough brainstorming. Instead of traditional annotator-based feedback labeling, we adopted the advice rankings based on majority votes from this forum as a proxy for Collective Intelligence~\cite{yang-etal-2023-rumor}, as illustrated in Figure~\ref{fig:Intro}. This novel approach enabled us to complete our benchmark, positioning AdvisorQA as a pioneering tool for harnessing collective intelligence in evaluating subjective advice.

% Large language models (LLMs)~\citep{openai2023gpt, touvron2023llama} have shown significant usefulness in enhancing human decision-making, holding the promise to revolutionize various fields such as healthcare~\citep{moor2023foundation, arora2023promise}, search~\citep{zelch2023commercialized}, and science~\citep{kung2023performance, lee2023qasa}. With this progress, there has been an emphasis on developing benchmarks that assess the `\textit{objective}' helpfulness of LLMs, evaluating their ability to provide \textit{accurate and factual} inference to posed challenges~\citep{hendrycks2020measuring, cobbe2021training, hwang2022multi, ye2023flask}.

% However, as LLMs' application extends into more nuanced interactions in daily life, there is a pronounced need for AI to advise personal decision-making regarding \textit{deeply personalized and subjective} issues that individuals face~\citep{casper2023open, kasneci2023chatgpt}. The complex nature of human concerns in such personalized contexts involves \textit{subjective} considerations, which are not sufficiently addressed by purely \textit{objective} evaluations~\citep{bolotova2022non, bolotova-baranova-etal-2023-wikihowqa}. This gap underlines the urgent need for a new benchmark to comprehensively evaluate LLMs' performance as personal advisors. In response, we introduce "AdvisorQA: A Benchmark for Advice-seeking Question Answering," a novel initiative designed to bridge this divide. AdvisorQA aims to 1) evaluate and 2) enhance the ability of LLMs to provide relevant and empathetic advice on deeply personal matters, as illustrated in Figure~\ref{fig:Intro}.

% Evaluating advice on deeply personal experiences presents formidable challenges~\citep{krishna-etal-2021-hurdles, casper2023open, weerasooriya-etal-2023-subjective}. Each question can elicit a range of subjective opinions, necessitating an assessment approach that extends beyond a limited number of annotators to collaborative brainstorming among individuals with diverse backgrounds~\citep{sandri-etal-2023-dont, fleisig-etal-2023-majority}. Furthermore, managing ethical issues emerging in the problem-solving process is crucial~\citep{lee-etal-2023-square, hendrycks2023aligning}. To navigate this complexity, we utilized the millions-user scale subreddit forum LifeProTips, a dynamic platform where individuals share advice on personal matters and engage in thorough brainstorming. Instead of traditional annotator-based feedback labeling, we adopted the advice rankings based on majority votes from this forum as a proxy for Collective Intelligence~\cite{yang-etal-2023-rumor}, as illustrated in Figure~\ref{fig:Intro}. This novel approach enabled us to complete our benchmark, positioning AdvisorQA as a pioneering tool for harnessing collective intelligence in evaluating subjective advice.

